How Far Can Camels Go? Exploring the State of Instruction Tuning on Open Resources

In this work we explore recent advances in instruction-tuning language models on a range of open instruction-following datasets. Despite recent claims that open models can be on par with state-of-the-art proprietary models, these claims are often accompanied by limited evaluation, making it difficult to compare models across the board and determine the utility of various resources. We provide a large set of instruction-tuned models from 6.7B to 65B parameters in size, trained on 12 instruction datasets ranging from manually curated (e.g., OpenAssistant) to synthetic and distilled (e.g., Alpaca) and systematically evaluate them on their factual knowledge, reasoning, multilinguality, coding, and open-ended instruction following abilities through a collection of automatic, model-based, and human-based metrics. We further introduce T\"ulu, our best performing instruction-tuned model suite finetuned on a combination of high-quality open resources. Our experiments show that different instruction-tuning datasets can uncover or enhance specific skills, while no single dataset (or combination) provides the best performance across all evaluations. Interestingly, we find that model and human preference-based evaluations fail to reflect differences in model capabilities exposed by benchmark-based evaluations, suggesting the need for the type of systemic evaluation performed in this work. Our evaluations show that the best model in any given evaluation reaches on average 87% of ChatGPT performance, and 73% of GPT-4 performance, suggesting that further investment in building better base models and instruction-tuning data is required to close the gap. We release our instruction-tuned models, including a fully finetuned 65B T\"ulu, along with our code, data, and evaluation framework at https://github.com/allenai/open-instruct to facilitate future research.

==> checklist.tex <==
\section*{NeurIPS Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}[leftmargin=*]

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See limitations section in supplementary materials.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See broader impacts section in supplementary materials.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Our github URL links to evaluation and training code with instructions on how to use.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{} See the instruction datasets details section in supplementary materials.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{Participants were all NLP researchers and were invited to voluntarily join the annotation effort. Participants could provide ongoing feedback through various means, including the interface itself.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{Participants were all employed in by the Authors' company, and performed annotation voluntarily as part of regular work duties.}
\end{enumerate}

\end{enumerate}

==> tables/average_perf.tex <==

\begin{table}[]
\caption{Average performance across MMLU, GSM, BBH, TyDiQA, Codex, and AlpacaFarm evaluations for \llama models of varying size trained on each dataset.}
\begin{tabular}{@{}ccccc@{}}
\hline
\textbf{Dataset ↓}       & \multicolumn{1}{l}{\textbf{7B}}         & \multicolumn{1}{l}{\textbf{13B}}        & \multicolumn{1}{l}{\textbf{30B}}        & \multicolumn{1}{l}{\textbf{65B}}        \\ \hline
SuperNI                   & \cellcolor[HTML]{FFFFFF}19.118          & \cellcolor[HTML]{F7FCF9}20.997          & -                                       & -                                       \\
CoT                       & \cellcolor[HTML]{D9F0E5}27.530          & \cellcolor[HTML]{BCE4D0}33.853          & -                                       & -                                       \\
Flan V2                   & \cellcolor[HTML]{DFF2E9}26.295          & \cellcolor[HTML]{CEEBDD}29.978          & -                                       & -                                       \\
Dolly                     & \cellcolor[HTML]{E5F5ED}24.888          & \cellcolor[HTML]{CAEADA}30.776          & -                                       & -                                       \\
Open Assistant 1          & \cellcolor[HTML]{D8EFE4}27.818          & \cellcolor[HTML]{ADDEC6}37.142          & -                                       & -                                       \\
Self-instruct (original)  & \cellcolor[HTML]{F6FCF9}21.103          & \cellcolor[HTML]{F4FBF7}21.658          & -                                       & -                                       \\
Unnatural Instructions    & \cellcolor[HTML]{EAF7F1}23.793          & \cellcolor[HTML]{DCF1E7}26.875          & -                                       & -                                       \\
Alpaca                    & \cellcolor[HTML]{D8EFE4}27.731          & \cellcolor[HTML]{CDEBDC}30.209          & -                                       & -                                       \\
Code-Alpaca               & \cellcolor[HTML]{DEF2E8}26.519          & \cellcolor[HTML]{C7E9D8}31.367          & -                                       & -                                       \\
GPT4-Alpaca               & \cellcolor[HTML]{C6E8D7}31.646          & \cellcolor[HTML]{AFDFC7}36.628          & -                                       & -                                       \\
Baize                     & \cellcolor[HTML]{DCF1E7}26.822          & \cellcolor[HTML]{CBEADB}30.635          & -                                       & -                                       \\
ShareGPT                  & \cellcolor[HTML]{C2E6D4}\textbf{32.584} & \cellcolor[HTML]{A3DABF}\textbf{39.345} & \cellcolor[HTML]{7ECBA5}\textbf{47.383} & \cellcolor[HTML]{67C295}\textbf{52.380} \\
\modelname{}  (\textit{Human-only mix}) & \cellcolor[HTML]{BDE5D1}33.606          & \cellcolor[HTML]{A1D9BE}39.704          & \cellcolor[HTML]{74C79E}49.574          & \cellcolor[HTML]{62C092}53.331          \\
\modelname{} (\textit{Human+GPT mix})  & \cellcolor[HTML]{A5DBC0}\textbf{38.817} & \cellcolor[HTML]{8BD0AE}\textbf{44.460} & \cellcolor[HTML]{5FBE8F}\textbf{54.131} & \cellcolor[HTML]{57BB8A}\textbf{55.690} \\ \hline
\end{tabular}
\end{table}

==> tables/complete_results.tex <==
\begin{table}[htbp]
\centering
\setlength\tabcolsep{4pt}
\caption{An overview of the performance of all models finetuned for this work, along with proprietary models, on selected benchmarks.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
\textbf{}                                                         & \textbf{\begin{tabular}[c]{@{}c@{}}MMLU \\ (factuality)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}GSM\\ (reasoning)\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}BBH \\ (reasoning)\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}TydiQA\\ (multiling.)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Codex-Eval\\ (coding)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}AlpacaFarm\\ (creative inst.)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Average\end{tabular}} \\ \midrule
\textbf{\begin{tabular}[c]{@{}c@{}}Metric\\ (Setup)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}EM\\ (0-shot)\end{tabular}}        & \textbf{\begin{tabular}[c]{@{}c@{}}EM\\ (8-shot, CoT)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}EM \\ (3-shot, CoT)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}F1\\ (1-shot, GP)\end{tabular}}          & \textbf{\begin{tabular}[c]{@{}c@{}}P@10\\ (0-shot)\end{tabular}}       & \textbf{\begin{tabular}[c]{@{}c@{}}Win \% vs \\ \instructgpt{003}\end{tabular}} &     \\ \midrule
\multicolumn{7}{c}{Proprietary models ↓}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \midrule
GPT-4-0314                                                        & 82.4                                                                  & 92.5                                                                & 88.0                                                                 & 70.8                                                                        & 94.1                                                                   & 93.2 & 86.8                                                                          \\
ChatGPT-turbo-0301                                                & 67.9                                                                  & 76.0                                                                & 66.1                                                                 & 51.9                                                                        & 88.4                                                                   & 83.0  & 72.2                                                                          \\ \midrule
\multicolumn{7}{c}{LLaMa 65B finetuning experiments ↓}                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \midrule
Vanilla LLaMa 65B                                                 & 58.7                                                                  & 50.5                                                                & \textbf{57.1}                                                        & \textbf{57.4}                                                                        & 42.9                                                                   & -      & -                                                                        \\
ShareGPT	& \textbf{61.5} & 42.0 & 52.1 & 33.5 & \textbf{53.5} & \textbf{72.8} & 52.6 \\
Tulu 65B (human-only data)                                        & 60.7                                                         & 57.5                                                                & 52.7                                                                 & 58.5                                                                        & 43.2                                                                   & 47.4        & 53.3                                                                   \\
Tulu 65B (human+GPT data)                                         & 59.2                                                                  & \textbf{60.0}                                                       & 53.5                                                                 & 51.8                                                                        & 45.9                                                                   & 63.8    & 55.7                                                              \\ \midrule
\multicolumn{7}{c}{LLaMa 30B finetuning experiments ↓}                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \midrule
Vanilla LLaMa 30B                                                 & 54.1                                                                  & 33.5                                                                & 48.5                                                                 & 57.5                                                                        & 42.9                                                                   & -   & -                                                                           \\
ShareGPT & 54.7 & 38.5 & \textbf{50.6} & 32.4 & 37.9 & \textbf{70.2} & 47.4 \\
Tulu 30B (human-only data)                                        & 56.3                                                                  & 49.5                                                                & 47.8                                                                 & \textbf{58.9}                                                                        & 39.4                                                                   & 45.5 & 49.6                                                                          \\
Tulu 30B (human+GPT data)                                         & \textbf{57.7}                                                                  & \textbf{51.0}                                                                & 48.7                                                                 & 58.2                                                                        & \textbf{46.0}                                                                   & 63.1     & 54.1                                                             \\ \midrule
\multicolumn{7}{c}{LLaMa 13B finetuning experiments ↓}                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \midrule
Vanilla LLaMa 13B                                                 & 42.5                                                                  & 14.0                                                                & 36.9                                                                 & 47.4                                                                        & 26.6                                                                   & -    & -                                                                          \\
SuperNI                                                           & 49.8                                                                  & 4.0                                                                 & 2.8                                                                  & \textbf{51.4}                                                               & 13.1                                                                   & 5.0       & 21.0                                                                     \\
CoT                                                               & 44.5                                                                  & \textbf{39.5}                                                       & 39.0                                                                 & 52.2                                                                        & 23.3                                                                   & 4.7         & 33.9                                                                   \\
Flan V2                                                           & \textbf{50.7}                                                         & 21.0                                                                & 39.2                                                                 & 47.5                                                                        & 16.2                                                                   & 5.3    &                                                                         \\
Dolly                                                             & 45.3                                                                  & 17.0                                                                & 26.0                                                                 & 46.8                                                                        & 31.4                                                                   & 18.3                                                                           \\
Open Assistant 1                                                  & 43.1                                                                  & 16.0                                                                & 38.5                                                                 & 38.3                                                                        & 31.8                                                                   & 55.2                                                                           \\
Self-instruct                                                     & 30.3                                                                  & 9.0                                                                 & 29.6                                                                 & 40.4                                                                        & 13.4                                                                   & 7.3                                                                            \\
Unnatural Instructions                                            & 46.2                                                                  & 7.5                                                                 & 32.8                                                                 & 39.3                                                                        & 24.8                                                                   & 10.8                                                                           \\
Alpaca                                                            & 45.1                                                                  & 8.0                                                                 & 34.5                                                                 & 32.8                                                                        & 27.6                                                                   & 33.2                                                                           \\
Code-Alpaca                                                       & 42.6                                                                  & 12.0                                                                & 36.6                                                                 & 41.3                                                                        & \textbf{34.5}                                                          & 21.3                                                                           \\
GPT4-Alpaca                                                       & 47.0                                                                  & 14.0                                                                & 38.3                                                                 & 24.4                                                                        & 32.5                                                                   & 63.6                                                                           \\
Baize                                                             & 43.5                                                                  & 8.5                                                                 & 36.7                                                                 & 33.9                                                                        & 27.3                                                                   & 33.9                                                                           \\
ShareGPT                                                          & 49.2                                                                  & 16.0                                                                & 40.1                                                                 & 30.1                                                                        & 31.6                                                                   & \textbf{69.1}                                                                  \\
Tulu 13B (human-only data)                                        & 50.4                                                                  & 36.5                                                                & 39.4                                                                 & 49.8                                                                        & 23.7                                                                   & 38.5                                                                           \\
Tulu 13B (human+GPT data)                                         & 49.2                                                                  & 36.5                                                                & \textbf{42.8}                                                        & 46.1                                                                        & 35.0                                                                   & 57.2                                                                           \\ \midrule
\multicolumn{7}{c}{LLaMa 7B finetuning experiments ↓}                                                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \midrule
Vanilla LLaMa 7B                                                  & 31.0                                                                  & 9.0                                                                 & 33.3                                                                 & 39.1                                                                        & 18.3                                                                   & -                                                                              \\
SuperNI                                                           & 44.1                                                                  & 4.0                                                                 & 1.9                                                                  & \textbf{47.9}                                                               & 11.7                                                                   & 5.2                                                                            \\
CoT                                                               & 41.3                                                                  & \textbf{27.5}                                                       & 31.3                                                                 & 44.4                                                                        & 17.3                                                                   & 3.4                                                                            \\
Flan V2                                                           & 45.4                                                                  & 13.0                                                                & 36.1                                                                 & 45.0                                                                        & 12.9                                                                   & 5.3                                                                            \\
Dolly                                                             & 38.0                                                                  & 7.0                                                                 & 24.4                                                                 & 43.6                                                                        & 22.1                                                                   & 14.4                                                                           \\
Open Assistant 1                                                  & 32.9                                                                  & 6.5                                                                 & 29.5                                                                 & 26.8                                                                        & 20.4                                                                   & 50.8                                                                           \\
Self-instruct (original)                                          & 35.7                                                                  & 6.5                                                                 & 29.2                                                                 & 35.4                                                                        & 12.1                                                                   & 7.6                                                                            \\
Unnatural Instructions                                            & 42.9                                                                  & 5.0                                                                 & 30.0                                                                 & 36.3                                                                        & 19.8                                                                   & 8.8                                                                            \\
Alpaca                                                            & 41.5                                                                  & 10.0                                                                & 31.8                                                                 & 31.2                                                                        & 22.0                                                                   & 29.9                                                                           \\
Code-Alpaca                                                       & 34.7                                                                  & 7.5                                                                 & 30.5                                                                 & 36.7                                                                        & \textbf{29.2}                                                          & 20.5                                                                           \\
GPT4-Alpaca                                                       & 42.6                                                                  & 10.0                                                                & 32.3                                                                 & 23.6                                                                        & 25.0                                                                   & 56.3                                                                           \\
Baize                                                             & 40.3                                                                  & 5.5                                                                 & 32.4                                                                 & 29.8                                                                        & 23.8                                                                   & 29.1                                                                           \\
ShareGPT                                                          & 44.3                                                                  & 9.5                                                                 & 32.6                                                                 & 25.5                                                                        & 21.6                                                                   & \textbf{62.1}                                                                  \\
Tulu 7B (human-only data)                                         & 44.5                                                                  & 27.0                                                                & \textbf{39.2}                                                        & 45.7                                                                        & \textbf{27.8}                                                          & 48.6                                                                           \\
Tulu 7B (human+GPT data)                                          & \textbf{46.2}                                                         & 26.5                                                                & 34.8                                                                 & 42.2                                                                        & 20.2                                                                   & 31.7                                                                          \\ \midrule
\multicolumn{7}{c}{Non-LLaMa 7B finetuning experiments ↓}  \\ \midrule
Pythia 6.9B          & 34.6                                                                                      & 15.5                                                                                    & 27.8                                                                                     & 33.4                                                                                            & 21.4                                                                                       & 9.3                                                                            & 23.7                                 \\
OPT 6.7B             & 34.9                                                                                      & 15.5                                                                                    & 27.9                                                                                     & 27.2                                                                                            & 7.9                                                                                        & 14.5                                                                           & 21.3                                 \\
\bottomrule
\end{tabular}
}
\label{tab:performance}
\end{table}













